The Rectangular Peg Problem

For every smooth Jordan curve $\gamma$ and rectangle $R$ in the Euclidean plane, we show that there exists a rectangle similar to $R$ whose vertices lie on $\gamma$. The proof relies on Shevchishin's theorem that the Klein bottle does not admit a smooth Lagrangian embedding in $\mathbb{C}^2$.

==> sections/scholium.tex <==

Let $\phi \colon [0, \infty) \rightarrow (0,\pi)$ be a smooth function, and consider the symplectomorphism
\[ S_\phi \colon \C^2 \rightarrow \C^2 \colon (z,r,\theta) \mapsto (z, r, \theta + \phi(r)) {\rm .} \]
Then $L_\phi = S_\phi(L)$ is a Lagrangian torus, invariant under $R_\pi$, and which intersects $L$ cleanly along $\gamma \times \{ 0 \}$.  The proofs we have given apply to this situation, telling us that we can smooth $L \cup L_\phi$ along $\gamma \times \{ 0 \}$ to an immersed Lagrangian torus $T$ such that $K = g(T)$ is a smoothly immersed Lagrangian Klein bottle, which we know is not embedded by Shevchishin's theorem.  The following porism is immediate.

\begin{scholium*}
	Define the subset $A(\gamma) \subset [0,\infty) \times (0,\pi)$ by requiring $(r, \theta) \in A(\gamma)$ if and only if $\gamma$ admits a rectangle of diagonal length $2r$ and aspect angle $\theta$.  Then $A(\gamma)$ is not disjoint from the graph of any smooth function $\phi \colon [0, \infty) \rightarrow (0,\pi)$. \qed
\end{scholium*}
